Ongoing Tracking of Engagement in Motor Learning

Teaching motor skills such as playing music, handwriting, and driving, can greatly benefit from recently developed technologies such as wearable gloves for haptic feedback or robotic sensorimotor exoskeletons for the mediation of effective human-human and robot-human physical interactions. At the heart of such teacher-learner interactions still stands the critical role of the ongoing feedback a teacher can get about the student's engagement state during the learning and practice sessions. Particularly for motor learning, such feedback is an essential functionality in a system that is developed to guide a teacher on how to control the intensity of the physical interaction, and to best adapt it to the gradually evolving performance of the learner. In this paper, our focus is on the development of a near real-time machine-learning model that can acquire its input from a set of readily available, noninvasive, privacy-preserving, body-worn sensors, for the benefit of tracking the engagement of the learner in the motor task. We used the specific case of violin playing as a target domain in which data were empirically acquired, the latent construct of engagement in motor learning was carefully developed for data labeling, and a machine-learning model was rigorously trained and validated.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> figures/RL-notes.tex <==
1. 
 Cognitive and emotional engagement while learning with VR: The perspective of multimodal methodology, 2022
 Ilana Dubovi - Tel Aviv

- Using: facial expression, eye tracking, EDA, and self reports
- Task: learning with VR
“only the facial expression data channel was able to detect fluctuations in engagement during the different learning session phases “
- using multimodal data channels encompassing different types of objective and subjective measures, can provide insights into a more holistic understanding of engagement in learning and learning achievements. 
- engagement in learning but not in motor learning
- defined: Engagement captures behavioral, emotional, and cognitive manifestations of student learning 
- Stemmed from Control Value Theory (CVT) according to which positive and negative emotions affect, sustain or disrupt, learner’s engagement.
- “until now most researchers have used self-reports or observations to measure engagement “
- positive and negative affect scale (PANAS) consisting of 20 items.

2. 
Learner Engagement Measurement and
Classification in 1:1 Learning, 2014
- using 2D/3D cameras and eye tracking, body posture, facial points, gaze
- analysis of emotions from camera, facial landmarks from 3D
- engagement while in general learning (high school students)
- engaged/not engaged labeling via video observations

3.
Measuring Learner Engagement in Computer-Equipped
College Classrooms, 2008

- classroom environment in college writing and computer-equipped classroom.
- engagement captures as a task property via computer-based behaviors (internet visits count) classifying between relevant and non relevant visits with respect to the classroom activity.
- manipulation was altering between interactive simulation task and a plain lecture.
- interactive task triggered higher relevant visits.

4.
EEG Correlates of Task Engagement and Mental Workload in Vigilance, Learning and Memory Tasks, 2007

- domain: operational environment for increased safety (e.g., military)
- uses EEG
- EEG was ‘objectively’ measured using conventional frequency bands derived from EEG power spectra (every 1 sec)
- Relationship with vigilance, workload, and task performance.
- Shows correspondence to information-gathering, visual scanning and sustained attention.
- HRV, GSR etc. may give indication of cognitive state changes but EEG is the only source that  gives reliable and accurate a millisecond timeframe.

5.
Measuring Cognitive Engagement: An Overview of Measurement Instruments and Techniques, 2021

- An exaughstive survey of different measures for cognitive engagement, catering 
- self-report scales, observations, interviews, teacher ratings, experience sampling, eye-tracking, physiological sensors, trace analysis, and content analysis. 

- Highlighting GSR, EMG for emotional and EEG for cognitive

6. 
Measuring Task Engagement as an Input to Physiological Computing, 2009

- Task engagement - a commitment to task goal conceived as a combined cognitive and emotional concept.
- employing EEG, pupilometry, and blood pressure.
- manipulating memory load via gradual increase of task difficulty and positive vs negative feedback.

7.
 Rethinking (Dis)engagement in human-computer interaction, 2022

- engagement as desirability with respect to user’s goals.
- highlighting a value also in capturing disengagement properly, sometimes even as a positive property of the user experience, as a potential signal for ceasing usage and taking a break.

8.
A wearables-based approach to detect and identify momentary engagement
in afterschool Makerspace programs, 2019

- maker learning for youth - creation of physical and digital artifacts.
- utilizing GSR and cameras
- identify moments of engagement
- The concept is also very much task oriented in its nature.

==> figures/docs/eafe990e-c27c-46b5-903c-7af2d051640e <==
{"id":"321241621323","lines":[{"id":"n0.3851416450923924","blocks":[],"style":{"align":"center"}},{"id":"n0.42803712142747985","blocks":[{"id":"n0.7909660440098397","text":"\\diagram","type":"composite","elements":{"de018936991804895498":{"id":"de018936991804895498","lines":[{"id":"n0.2497640979335769","blocks":[{"id":"n0.48883865766797374","text":"Windowing"}]},{"id":"n0.5124074108171436","blocks":[{"id":"n0.2865013965165134","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.024955607170010774","lines":[{"id":"n0.902517351287711","blocks":[{"id":"n0.7278091855264008","text":"& "}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}},{"text":"Feature","id":"n0.6103619198218532"}],"style":null},{"id":"n0.3349312004190901","blocks":[{"id":"n0.10005613381807432","text":"Extraction"}],"style":null}],"shape":{"data":{"p":{"x":117,"y":33}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true,"isInGroup":true},"de396911194519339":{"id":"de396911194519339","lines":[{"blocks":[{"id":"n0.35447971058862304","text":"Raw"}],"id":"n0.010357142378850215"},{"id":"n0.17008944264464965","blocks":[{"id":"n0.33790477035742816","text":"Sensor"}],"style":null},{"id":"n0.8720162564918545","blocks":[{"id":"n0.2376142337370687","text":"Data"}],"style":null}],"shape":{"data":{"p":{"x":13,"y":31}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true,"isInGroup":true},"de38091119372357496":{"id":"de38091119372357496","lines":[{"blocks":[{"id":"n0.5794533246572301","text":"Predict"}],"id":"n0.8898485646074163"},{"id":"n0.9592154889217934","blocks":[{"id":"n0.1593976753514652","text":"Discomfort"}],"style":null}],"shape":{"data":{"p":{"x":245,"y":50}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true,"isInGroup":true},"de8119064312976849":{"id":"de8119064312976849","lines":[{"blocks":[{"text":"Predict","id":"n0.05828151093225897"}],"id":"n0.5506404099523997"},{"blocks":[{"id":"n0.31170703735212035","text":"Engagement"}],"style":null,"id":"n0.8034828597628288"}],"shape":{"data":{"p":{"x":355,"y":139}},"anchor":"left-top","settings":{"fontSize":"\\small"}},"isTextMode":true,"isInGroup":true},"de9902810701118417":{"id":"de9902810701118417","lines":[{"id":"n0.3168322085721338","blocks":[{"id":"n0.30947984847108423","text":"not engaged"}]}],"shape":{"data":{"p":{"x":563,"y":156}},"anchor":"left-top"},"isTextMode":true},"de5966388579097124":{"id":"de5966388579097124","lines":[{"id":"n0.11326637578767573","blocks":[{"id":"n0.7247517198689731","text":"engaged"}]}],"shape":{"data":{"p":{"x":539,"y":135}},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di25868853331498753","items":[],"style":{}},"shapes":[{"id":"dg12289226506737583","entities":[{"id":"dp21299074500456994","type":"doc-rounded-rect","data":{"p1":{"x":116,"y":10},"p2":{"x":190,"y":113}}},{"id":"da7395819321049393","data":[{"x":64,"y":99},{"x":116,"y":99}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da19355084286230584","data":[{"x":64,"y":24},{"x":116,"y":24}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da4280670756062025","data":[{"x":64,"y":80.25},{"x":116,"y":80.25}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da01644034709378328","data":[{"x":64,"y":61.5},{"x":116,"y":61.5}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da6784973043185042","data":[{"x":64,"y":42.75},{"x":116,"y":42.75}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da7945294531024377","data":[{"x":191,"y":99},{"x":243,"y":99}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da20001104063754593","data":[{"x":191,"y":24},{"x":243,"y":24}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da7824119692722447","data":[{"x":191,"y":80.25},{"x":243,"y":80.25}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da8042508050252782","data":[{"x":191,"y":61.5},{"x":243,"y":61.5}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da3308959932479949","data":[{"x":191,"y":42.75},{"x":243,"y":42.75}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dp20548466314882974","type":"doc-rounded-rect","data":{"p1":{"x":243,"y":10.800000000000011},"p2":{"x":317,"y":113.80000000000001}}},{"id":"da6418530510712965","data":[{"p1":{"x":217,"y":42.75},"p2":{"x":352,"y":150.35000000000002},"cp":{"dx":-2,"dy":123},"cp2":{"dx":-138,"dy":-0.6000000000000227}}],"head":">","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"dp6486726369098613","type":"doc-rounded-rect","data":{"p1":{"x":352,"y":95},"p2":{"x":440,"y":219.8}}},{"id":"da5545473710144997","data":[{"p1":{"x":211,"y":62},"p2":{"x":352,"y":169},"cp":{"dx":-2,"dy":123},"cp2":{"dx":-138,"dy":-0.6000000000000227}}],"head":">","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da41785951251706943","data":[{"p1":{"x":204,"y":81},"p2":{"x":351,"y":187},"cp":{"dx":-2,"dy":123},"cp2":{"dx":-138,"dy":-0.6000000000000227}}],"head":">","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da3684251131235262","data":[{"p1":{"x":198,"y":99},"p2":{"x":352,"y":205},"cp":{"dx":-2,"dy":123},"cp2":{"dx":-138,"dy":-0.6000000000000227}}],"head":">","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da5516193080492896","data":[{"p1":{"x":224,"y":24},"p2":{"x":352,"y":131.60000000000002},"cp":{"dx":-2,"dy":123},"cp2":{"dx":-138,"dy":-0.6000000000000227}}],"head":">","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da2080171214764559","data":[{"p1":{"x":317,"y":59},"p2":{"x":352,"y":115},"cp":{"dx":30,"dy":3},"cp2":{"dx":-50,"dy":2}}],"head":">","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"dl11989599644672733","linkedId":"de018936991804895498"},{"id":"dl2813305371588054","linkedId":"de396911194519339"},{"id":"dl6319714715366755","linkedId":"de38091119372357496"},{"id":"dl8186112844789389","linkedId":"de8119064312976849"}]},{"id":"da01734908720942896","data":[{"x":440,"y":159},{"x":476,"y":159.5}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dp22052104704643882","type":"generic-shape","data":{"p1":{"x":479,"y":148.5},"p2":{"x":559,"y":169}},"subType":"pulse-1"}],"settings":{"grid":true,"diagramHeight":231}}]},{"id":"n0.8789959300393606","blocks":[],"style":{"align":"center"}}],"pageSettings":{"pageSize":{"width":700}},"delayRenderCache":{"av":190,"map":{}},"___version":2,"version":2,"av":190}
